Techniques for Inverted Index Compression

The data structure at the core of large-scale search engines is the inverted index, which is essentially a collection of sorted integer sequences called inverted lists. Because of the many documents indexed by such engines and stringent performance requirements imposed by the heavy load of queries, the inverted index stores billions of integers that must be searched efficiently. In this scenario, index compression is essential because it leads to a better exploitation of the computer memory hierarchy for faster query processing and, at the same time, allows reducing the number of storage machines. The aim of this article is twofold: first, surveying the encoding algorithms suitable for inverted index compression and, second, characterizing the performance of the inverted index through experimentation.

==> entropy.tex <==
\subsection{Arithmetic}\label{subsec:arithmetic}
The first concept of Arithmetic coding was introduced by Elias before
1963 according to Note 1 on page 61 in the book by~\citet*{abramson1963information}.
However, the method requires infinite precision arithmetic and,
because of this, it remained unpublished.
The first practical implementation
were designed during 1976 by~\citet*{rissanen1976generalized} and~\citet*{pasco1976source},
and later refined by~\citet*{rissanen1979arithmetic}.

This method offers higher compression ratios with respect to Huffman,
especially on highly skewed distributions,
because it is not a prefix-free code, so it does not require at least
one bit to encode a symbol. Indeed a single bit may correspond to more
than one input symbol.
However, Huffman codes are faster to decode; Arithmetic does not permit
to decode an output stream starting from an arbitrary position, but only
sequential decoding is possible.

Given a sequence of symbols $\seq = s_1s_2...s_n$, the main idea behind the method works as follows.
The interval $[0,1)$ is partitioned into $|\Sigma|$ segments of length proportional to the probabilities of the symbols.
Then the subinterval corresponding with $s_1$, say $[\ell_1, r_1)$, is chosen and the partitioning step is applied to it.
The process stops when all input symbols have been considered, thus
after $n$ steps, and outputs a single real number $x$ in $[\ell_n, r_n)$,
that is the interval associated to the last input symbol $s_n$.
Then the pair $(x, n)$ suffices to decode the original input sequence $\seq$.
Fig.~\ref{fig:arithmetic} shows an encoding example for the sequence $\seq = abbaac$, with $\pr(a) = 1/2$, $\pr(b) = 1/3$ and $\pr(c) = 1/6$.

\begin{figure}
\centering
\includegraphics[scale=0.7]{{figures/arithmetic}}
\caption{Arithmetic coding example applied to the input sequence $abbacc$.
The final interval is $\Big[\frac{149}{432},\frac{25}{72}\Big)$.}
\label{fig:arithmetic}
\end{figure}

It can be shown that Arithmetic coding takes at most $nH_0 + 2$ bits to encode
a sequence $\seq$ of length $n$. This means that the overhead with respect to
the empirical entropy $H_0$ is only of $2/n$ bits per symbol, thus negligible
for basically all practical values of $n$.
As already pointed out, Arithmetic coding requires infinite precision that can
be very costly to be approximated. In fact, a practical implementation~\cite{witten1987arithmetic} using
approximated arithmetic can take up to $nH_0 + \frac{2}{100}n$ bits, thus
having $0.02$ bits of loss per symbol rather than $2/n$.

\subsection{Asymmetric numeral systems}\label{subsec:ANS}
\emph{Asymmetric numeral systems} ({\ans}) is a family of entropy coding algorithms,
originally developed by~\citet*{duda09,duda13}, which approaches the compression ratio
of Arithmetic coding with a decompression speed comparable with the one of Huffman~\cite{duda15}.

The basic idea of {\ans} coding is to represent a \emph{sequence}
of symbols with a natural number $x$.
In general, if each symbol $s$ is a bit, then appending $s$ to the end of the binary string
representing $x$ will generate a new integer $x^\prime = 2x + s$.
This code is optimal whenever $\mathbb{P}(0) = \mathbb{P}(1) = 1/2$.
{\ans} generalizes this fact by adapting it to a general distribution of symbols.
In this case, appending a symbol $s$ to $x$ increases the information content
from $\log_2 x $ bits to $\log_2 x - \log_2 \pr(s) = \log_2 (x/\pr(s))$ bits,
thus the new generated natural number will be $x^\prime \approx x/\pr(s)$.

\begin{figure}
\centering
\subfloat[]{
	\scalebox{0.8}{
    \input{tables/ans1.tex}}
    \label{fig:ans1}
}
\subfloat[]{
	\scalebox{0.8}{
    \input{tables/ans2.tex}}
    \label{fig:ans2}
}

\caption{Two example of {\ans} encoding table, with respectively frame $f[1..6] = [aaabbc]$ and $f[1..4] = [caba]$.}
\end{figure}

Let us consider a more concrete example~\cite{ANS2}, with an alphabet of 3 symbols only,
namely $\{a,b,c\}$ assuming $\pr(a)=1/2$, $\pr(b)=1/3$ and $\pr(c)=1/6$.
In order to derive the encoding of a sequence of symbols, a \emph{frame} $f[1..m]$
of symbols is constructed, having $1/2$ of the entries equal to $a$, $1/3$ equal to $b$ and $1/6$
equal to $c$.
For example, one such frame could be $f[1..6] = [aaabbc]$, but other symbol permutations
with possibly larger $m$ are possible as well.
The frame determines a table that is used to map
a sequence of symbols to an entry in the table.
Refer to Fig.~\ref{fig:ans1} for an example with a frame $f[1..6] = [aaabbc]$.
The entries in the table are the natural numbers assigned incrementally in the order determined
by the frame. For example, since the first three symbols in the frame are $aaa$, the first numbers
assigned to $a$'s row are 1,2 and 3. The next two symbols are $bb$, so $b$'s row gets 4 and 5.
The last symbol in the frame is $c$, so the first entry in $c$'s row is 6.
The process now proceed in cycles, thus placing 7, 8 and 9 in $a$'s row; 10 and 11 in $b$'s row,
a final 12 in $c$'s row, and so on (first 10 columns are shown in the figure).
Fig.~\ref{fig:ans2} shows an example for another distribution of the symbols, constructed
using a frame $f[1..4] = [caba]$.

Now, consider the sequence $caa$ and let us determine its {\ans} code with the table
in Fig.~\ref{fig:ans1}. We make use of the \emph{transition function} defined by the table $T$
itself as $\var{state}^{\prime} = T[s, \var{state}]$ which, given a symbol $s$ and a \var{state} value,
produces the next $\var{state}^{\prime}$ of the encoder.
At the beginning we set $\var{state} = 0$, thus for the given sequence $caa$ the \var{state} variable
assumes values $0 \rightarrow 6 \rightarrow 13 \rightarrow 26$ (last value not shown in the figure).
The code assigned to the sequence is, therefore, the integer 26.
For the sequence $acb$ under the encoding table in Fig.~\ref{fig:ans2} we generate, instead,
the transitions $0 \rightarrow 2 \rightarrow 9 \rightarrow 39$, thus the assigned code is 39.
Decoding reverts this process. For example, given 39 we know that the last symbol of the encoded
sequence must have been $b$ because 39 is found on the second row of the table. The value
is in column 9, which is found in column 2 in the third row that corresponds to the $c$ symbol.
Finally, the column number 2 is found in $a$'s row, thus we emit the message $acb$.


==> intersection.tex <==
\SetArgSty{textnormal}
\begin{algorithm}[H]
\SetKwBlock{Begin}{}{}
\Begin(\func{intersect}\text{($\seq_0,\ldots,\seq_{k-1}$)})
{
	$\var{results} = 0$ \\
	$\var{candidate} = \seq_0[0]$ \\
	$i = 1$ \\
	\While{$\var{candidate} <$ \text{{\#} of documents}}{
		\For{$;$ $i < k;$ $i = i + 1$}{
			$z = \seq_i.$\func{\Nextgeq}$(\var{candidate})$ \\
			\If{$z$ \text{!=} $\var{candidate}$}{
				$\var{candidate} = z$ \\
				$i = 0$ \\
				\code{break} \\
			}
		}
	
		\If{$i == k$}{
			$\var{results} = \var{results} + 1$ \\
			$\var{candidate} = \seq_0.$\func{\Nxt} \\
			$i = 1$ \\
		}
	}
	\code{return} $\var{results}$ \\
}
\end{algorithm}

==> tables/AND_and_OR.tex <==
\begin{tabular}{l SS l SS l SS}
\toprule

Method
& \multicolumn{2}{c}{\gov}
&
& \multicolumn{2}{c}{\clue}
&
& \multicolumn{2}{c}{\cc}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){5-6}
\cmidrule(lr){8-9}

& {\AND} & {\OR}
&
& {\AND} & {\OR}
&
& {\AND} & {\OR}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){5-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){9-9}

{\vb}
& 3.20418 & 63.3809
&
& 14.5251 & 178.789
&
& 25.7834 & 165.1133
%& 2.080 & 5.475
%&
%& 10.515 & 17.676
%&
%& 15.911 & 22.257
\\

{\optvb}
%& 2.488 & 6.815
%&
%& 12.223 & 22.770
%&
%& 17.835 & 27.164
& 3.52606 & 70.2324
&
& 15.9411 & 198.449
&
& 26.4869 & 177.635
\\

{\interp}
%& 7.900 & 16.104
%&
%& 40.141 & 56.115
%&
%& 60.574 & 74.825
& 12.5146 & 105.918
&
& 58.516 & 315.718
&
& 93.685 & 306.639
\\

{\cdelta}
%& 5.035 & 12.836
%&
%& 25.622 & 38.775
%&
%& 36.505 & 47.358
& 7.17108 & 90.2643
&
& 33.2689 & 247.45
&
& 53.2631 & 229.721
\\

%{\textsf{Opt-}\cdelta}
%& 15.3838 & 96.2982
%&
%& 49.5067 & 257.217
%&
%& 48.6601 & 227.873
%\\

{\rice}
& 6.20308 & 80.6013
&
& 28.787 & 222.215
&
& 46.1679 & 203.404
\\

{\opt}
%& 2.475 & 6.360
%&
%& 12.540 & 23.202
%&
%& 19.717 & 29.648
& 3.32847 & 69.002
&
& 15.2646 & 206.408
&
& 26.6338 & 192.56
\\

{\dint}
%& 2.507 & 6.175
%&
%& 12.170 & 21.481
%&
%& 18.892 & 27.246
& 3.65508 & 64.7154
&
& 17.1191 & 185.979
&
& 28.8337 & 172.461
\\

{\opf}
%& 2.810 & 6.541
%&
%& 14.780 & 22.953
%&
%& 20.368 & 27.496
& 4.00041 & 59.3138
&
& 18.7446 & 175.402
&
& 29.0913 & 162.967
\\

{\simples}
%& 2.860 & 6.700
%&
%& 14.628 & 22.749
%&
%& 21.558 & 28.735
& 4.16413 & 66.9295
&
& 19.3071 & 191.324
&
& 31.0128 & 177.062
\\

{\qmx}
& 2.86601 & 66.8876
&
& 12.9214 & 185.5
&
& 21.9784 & 166.013
\\

{\roaropt}
%& 0.316 & 1.350
%&
%& 1.641 & 5.403
%&
%& 1.285 & 4.600
& 0.722345 & 4.042857
&
& 2.967807 & 10.968146
&
& 2.562512 & 9.286689
\\

{\slice}
%& 0.321 & 1.607
%&
%& 1.673 & 6.277
%&
%& 1.78 & 7.252
& 1.11638 & 5.85409
&
& 4.88303 & 17.0359
&
& 4.59651 & 15.6504
\\

\bottomrule
\end{tabular}

==> tables/access_and_nextgeq.tex <==
\begin{tabular}{l rr l rr l rr}
\toprule

Method
& \multicolumn{2}{c}{\gov}
&
& \multicolumn{2}{c}{\clue}
&
& \multicolumn{2}{c}{\cc}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){5-6}
\cmidrule(lr){8-9}

& {\access} & {\Nextgeq}
&
& {\access} & {\Nextgeq}
&
& {\access} & {\Nextgeq}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){5-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){9-9}

{\vb}
& 150 & 185
&
& 180 & 216
&
& 203 & 240
\\

{\optvb}
& {\e} & {\e}
&
& {\e} & {\e}
&
& {\e} & {\e}
\\

{\interp}
& 1120 & 1105
&
& 1155 & 1145
&
& 1312 & 1290
\\

{\cdelta}
& 600 & 634
&
& 624 & 657
&
& 680 & 715
\\

{\opt}
& 110 & 132
&
& 117 & 138
&
& 75 & 93
\\

{\dint}
& {\e} & {\e}
&
& {\e} & {\e}
&
& {\e} & {\e}
\\

{\opf}
& 247 & 283
&
& 295 & 330
&
& 236 & 272
\\

{\simples}
& 273 & 307
&
& 325 & 357
&
& 325 & 359
\\

{\roaropt}
& 880 & 74
&
& 2291 & 84
&
& 597 & 92
\\

{\slice}
& 81 & 67
&
& 72 & 67
&
& 88 & 76
\\

\bottomrule
\end{tabular}

==> tables/access_queries.tex <==
\begin{tabular}{c rrr l rrr l rrr}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 195 & 174 & 240
&
& 155 & 184 & 222
&
& 105 & 151 & 189
\\

{\uniform}
& 118 & 122 & 173
&
& 88 & 103 & 123
&
& 58 & 75 & 86
\\

{\interp}
& 890 & 835 & 1295
&
& 904 & 960 & 1230
&
& 685 & 876 & 1062
\\

{\opt}
& 154 & 171 & 210
&
& 118 & 145 & 126
&
& 77 & 100 & 72
\\

{\roar}
& 475 & 545 & 610
&
& 294 & 453 & 402
&
& 111 & 365 & 310
\\

{\roaropt}
& 5604 & 18710 & 2852
&
& 2151 & 7681 & 1221
&
& 443 & 2254 & 612
\\

{\slice}
& 153 & 170 & 244
&
& 105 & 116 & 152
&
& 55 & 61 & 78
\\

\bottomrule
\end{tabular}

==> tables/and_queries.tex <==
\begin{tabular}{c rrr l rrr l rrr}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 3648 & 6671 & 16954
&
& 710 & 1591 & 3732
&
& 40 & 214 & 523
\\

{\uniform}
& 4652 & 8356 & 22818
&
& 856 & 1700 & 4455
&
& 40 & 192 & 530
\\

{\interp}
& 12169 & 23608 & 58349
&
& 2649 & 6377 & 14765
&
& 160 & 905 & 2323
\\

{\opt}
& 4380 & 7920 & 21710
&
& 826 & 1640 & 4185
&
& 40 & 190 & 490
\\

{\roar}
& 377 & 598 & 1138
&
& 99 & 232 & 353
&
& 10 & 57 & 98
\\

{\roaropt}
& 503 & 962 & 1338
&
& 128 & 331 & 395
&
& 13 & 75 & 115
\\

{\slice}
& 507 & 1080 & 2370
&
& 135 & 378 & 820
&
& 11 & 60 & 159
\\

\bottomrule
\end{tabular}

==> tables/centered.tex <==
\begin{tabular}{ccccccccccccc}
\toprule

0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\

\cmidrule(lr){1-13}

\textbf{\bit{0}}   & \textbf{\bit{0}}   & \textbf{\bit{0}}   & \textbf{\bit{0}}   & \textbf{\bit{0}}   & --        & --      & --      & \textbf{\bit{1}}  & \textbf{\bit{1}}   & \textbf{\bit{1}}   & \textbf{\bit{1}}   & \textbf{\bit{1}} \\
\bit{0}   & \bit{0}   & \bit{0}   & \bit{0}   & \bit{1}   & \bit{1}   & \bit{1} & \bit{1} & \bit{0}  & \bit{0}    & \bit{0}   & \bit{0}   & \bit{1} \\
\bit{0}   & \bit{0}   & \bit{1}   & \bit{1}   & \bit{0}   & \bit{0}   & \bit{1} & \bit{1} & \bit{0}  & \bit{0}    & \bit{1}   & \bit{1}   & \bit{0} \\
{\bit{0}} & {\bit{1}} & {\bit{0}} & {\bit{1}} & {\bit{0}} & \bit{1}   & \bit{0} & \bit{1} & {\bit{0}} & {\bit{1}} & {\bit{0}} & {\bit{1}} & {\bit{0}} \\

\bottomrule
\end{tabular}


==> tables/clueweb09.entropy.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $49.86$ & $25.01$\\

$512$ & $48.17$ & $24.16$\\

$1024$ & $47.77$ & $23.96$\\

$2048$ & $47.31$ & $23.73$\\

$4096$ & $46.76$ & $23.45$\\

$8192$ & $46.08$ & $23.11$\\

$16384$ & $45.31$ & $22.72$\\

$32768$ & $44.35$ & $22.24$\\
\bottomrule
\end{tabular}


==> tables/clueweb09.entropy.freqs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $2.79$ & $1.40$\\

$512$ & $2.63$ & $1.32$\\

$1024$ & $2.59$ & $1.30$\\

$2048$ & $2.53$ & $1.27$\\

$4096$ & $2.47$ & $1.24$\\

$8192$ & $2.39$ & $1.20$\\

$16384$ & $2.28$ & $1.15$\\

$32768$ & $2.13$ & $1.07$\\
\bottomrule
\end{tabular}


==> tables/clueweb09.gaps_entropy.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $9.40$ & $4.72$\\

$512$ & $8.21$ & $4.12$\\

$1024$ & $8.02$ & $4.02$\\

$2048$ & $7.82$ & $3.92$\\

$4096$ & $7.59$ & $3.80$\\

$8192$ & $7.32$ & $3.67$\\

$16384$ & $7.03$ & $3.52$\\

$32768$ & $6.68$ & $3.35$\\
\bottomrule
\end{tabular}


==> tables/clueweb09.gaps_logs.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $5.48$ & $2.75$\\

$512$ & $4.62$ & $2.32$\\

$1024$ & $4.50$ & $2.26$\\

$2048$ & $4.38$ & $2.19$\\

$4096$ & $4.23$ & $2.12$\\

$8192$ & $4.07$ & $2.04$\\

$16384$ & $3.89$ & $1.95$\\

$32768$ & $3.68$ & $1.85$\\
\bottomrule
\end{tabular}


==> tables/clueweb09.space.tex <==
\begin{tabular}{lrrrrrr}
\toprule

& \multicolumn{2}{@{}c@{}}{\textsf{space}} 
& \multicolumn{2}{@{}c@{}}{{\docs}} 
& \multicolumn{2}{@{}c@{}}{{\freqs}} \\

& \multicolumn{2}{@{}c@{}}{[{\total}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} \\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

{\bic}& $14.01$ & & $5.15$ & & $1.87$ & \\

\cmidrule(lr){2-7}

{\pef}
& $15.94$ & \color{DarkGray}{$(+14\%)$}
& $5.85$ & \color{DarkGray}{$(+14\%)$}
& $2.20$ & \color{DarkGray}{$(+18\%)$}\\

%{\CPEF}
%& $15.33$ & \color{DarkGray}{$(+9\%)$}
%& $5.54$ & \color{DarkGray}{$(+8\%)$}
%& $2.19$ & \color{DarkGray}{$(+17\%)$}\\
%
%{\ans}
%& $14.47$ & \color{DarkGray}{$(+3\%)$}
%& $5.36$ & \color{DarkGray}{$(+4\%)$}
%& $1.94$ & \color{DarkGray}{$(+4\%)$}\\

{\pfor}
& $17.15$ & \color{DarkGray}{$(+22\%)$}
& $6.18$ & \color{DarkGray}{$(+20\%)$}
& $2.41$ & \color{DarkGray}{$(+29\%)$}\\

{\cgamma}
& $17.41$ & \color{DarkGray}{$(+24\%)$}
& $6.52$ & \color{DarkGray}{$(+27\%)$}
& $2.20$ & \color{DarkGray}{$(+18\%)$}\\

{\cdelta}
& $16.98$ & \color{DarkGray}{$(+21\%)$}
& $6.05$ & \color{DarkGray}{$(+18\%)$}
& $2.46$ & \color{DarkGray}{$(+32\%)$}\\

{\simplee}
& $21.58$ & \color{DarkGray}{$(+54\%)$}
& $7.36$ & \color{DarkGray}{$(+43\%)$}
& $3.47$ & \color{DarkGray}{$(+86\%)$}\\

{\simplen}
& $20.41$ & \color{DarkGray}{$(+46\%)$}
& $7.23$ & \color{DarkGray}{$(+40\%)$}
& $3.01$ & \color{DarkGray}{$(+61\%)$}\\

{\simples}
& $19.36$ & \color{DarkGray}{$(+38\%)$}
& $6.92$ & \color{DarkGray}{$(+34\%)$}
& $2.79$ & \color{DarkGray}{$(+49\%)$}\\

{\qmx}
& $23.44$ & \color{DarkGray}{$(+67\%)$}
& $8.01$ & \color{DarkGray}{$(+56\%)$}
& $3.75$ & \color{DarkGray}{$(+101\%)$}\\

{\vb}
& $35.63$ & \color{DarkGray}{$(+154\%)$}
& $9.91$ & \color{DarkGray}{$(+92\%)$}
& $8.01$ & \color{DarkGray}{$(+329\%)$}\\

{\optvb}
& $17.88$ & \color{DarkGray}{$(+28\%)$}
& $6.54$ & \color{DarkGray}{$(+27\%)$}
& $2.48$ & \color{DarkGray}{$(+33\%)$}\\

{\varigb}
& $42.23$ & \color{DarkGray}{$(+201\%)$}
& $11.43$ & \color{DarkGray}{$(+122\%)$}
& $9.80$ & \color{DarkGray}{$(+425\%)$}\\

{\varigiu}
& $39.43$ & \color{DarkGray}{$(+181\%)$}
& $10.84$ & \color{DarkGray}{$(+111\%)$}
& $8.99$ & \color{DarkGray}{$(+381\%)$}\\

\bottomrule
\end{tabular}


==> tables/dac.tex <==
\begin{tabular}{ccccccccc}
\toprule
$B_1$ & \bit{0} & \bit{0} & \bit{1} & \bit{0} & \bit{1} & \bit{1} & \bit{1} & \bit{1} \\
$C_1$ & \bit{010} & \bit{111} & \bit{100} & \bit{101} & \bit{101} & \bit{110} & \bit{011} & \bit{001} \\
\cmidrule(lr){1-9}
$B_2$ & \bit{0} & \bit{0} & \bit{1} & \bit{0} & \bit{1} & & & \\
$C_2$ & \bit{001} & \bit{001} & \bit{001} & \bit{110} & \bit{000} & & & \\
\cmidrule(lr){1-9}
$B_3$ & \bit{0} & \bit{0} & & & & & & \\
$C_3$ & \bit{010} & \bit{010} & & & & & & \\
\bottomrule
\end{tabular}

==> tables/datasets.by_varying_density.tex <==
\begin{tabular}{c l r r r}
\toprule

Density & Statistic & {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}

\multirow{3}{*}{$10^{-2}$}
& Lists
  & \num{3513}
  & \num{5802}
  & \num{5930}
  \\

& Integers
  & \num{4347653438}
  & \num{11676154022}
  & \num{16677342102}   
  \\

& \%
  & 76
  & 74
  & 83
  \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}

\multirow{3}{*}{$10^{-3}$}
& Lists
  & \num{13276}
  & \num{21924}
  & \num{23085}
  \\

& Integers
  & \num{5066748826}
  & \num{13864451283}
  & \num{18969946075}   
  \\

& \%
  & 88
  & 87
  & 94
  \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}

\multirow{3}{*}{$10^{-4}$}
& Lists
  & \num{85893}
  & \num{99227}
  & \num{79954}
  \\

& Integers
  & \num{5390038277}
  & \num{14805194135}
  & \num{19681352639}  
  \\

& \%
  & 94
  & 93
  & 98
  \\
  
\bottomrule
\end{tabular}

==> tables/datasets.tex <==
\begin{tabular}{l r r r}
\toprule

Statistic & {\gov} & {\clue}  & {\cc} \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}

Lists
  & \num{35636425}
  & \num{92094694}
  & \num{43844574}
  \\
  
Universe
  & \num{24622347}
  & \num{50131015}
  & \num{43530315}
  \\

Integers
  & \num{5742630292}
  & \num{15857983641}
  & \num{20150335440}  
  \\
  
\bottomrule
\end{tabular}

==> tables/decoding.tex <==
%\sisetup{round-precision = 3}
\begin{tabular}{c SSS l SSS l SSS}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 0.513518 & 0.606247 & 0.528292
&
& 0.550443 & 0.662528 & 0.58574
&
& 0.582142 & 0.706762 & 0.618797
\\

{\uniform}
& 0.874415 & 1.28632 & 1.36301
&
& 0.941314 & 1.34128 & 1.41179
&
& 0.980144 & 1.35715 & 1.42167
\\

{\interp}
& 5.26176 & 6.7332 & 7.70933
&
& 5.54049 & 6.94862 & 7.8628
&
& 5.7008 & 7.00913 & 7.90128
\\

{\opt}
& 0.784609 & 1.14684 & 1.34422
&
& 0.857179 & 1.2216 & 1.48046
&
& 0.912888 & 1.25357 & 1.5303
\\

{\roar}
& 0.532040 & 0.716252 & 0.682651
&
& 0.525104 & 0.697586 & 0.685258
&
& 0.537158 & 0.706256 & 0.687055
\\

{\roaropt}
& 0.552781 & 0.755715 & 0.702587
&
& 0.548563 & 0.760792 & 0.690020
&
& 0.573709 & 0.776009 & 0.699855
\\

{\slice}
& 0.563091 & 0.670121 & 0.652603
&
& 0.571514 & 0.68987 & 0.673231
&
& 0.598734 & 0.725803 & 0.706615
\\

\bottomrule
\end{tabular}

==> tables/english_alphabet1.tex <==
\begin{tabular}{c c r r}
\toprule

symbol & probability & {\sf SF} & {\sf H} \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}

\sf A & 0.08833 & 010 & 1111 \\
\sf B & 0.01267 & 111110 & 100000 \\
\sf C & 0.02081 & 111010 & 00000 \\
\sf D & 0.04376 & 10111 & 11101 \\
\sf E & 0.14878 & 000 & 110 \\
\sf F & 0.02455 & 11011 & 00011 \\
\sf G & 0.01521 & 111100 & 100001 \\
\sf H & 0.05831 & 1001 & 0111 \\
\sf I & 0.05644 & 1010 & 0110 \\
\sf J & 0.00080 & 1111111110 & 0001010111 \\
\sf K & 0.00867 & 11111110 & 0001011 \\
\sf L & 0.04124 & 11000 & 11100 \\
\sf M & 0.02361 & 11100 & 00001 \\

\bottomrule
\end{tabular}


==> tables/english_alphabet2.tex <==
\begin{tabular}{c c r r}
\toprule

symbol & probability & {\sf SF} & {\sf H} \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}

\sf N & 0.06498 & 1000 & 1001 \\
\sf O & 0.07245 & 0110 & 1011 \\
\sf P & 0.02575 & 11010 & 01000 \\
\sf Q & 0.00080 & 11111111110 & 000101010 \\
\sf R & 0.06872 & 0111 & 1010 \\
\sf S & 0.05537 & 10110 & 0101 \\
\sf T & 0.09351 & 001 & 001 \\
\sf U & 0.02762 & 11001 & 01001 \\
\sf V & 0.01160 & 1111110 & 000100 \\
\sf W & 0.01868 & 111011 & 100011 \\
\sf X & 0.00146 & 111111110 & 00010100 \\
\sf Y & 0.01521 & 111101 & 100010 \\
\sf Z & 0.00053 & 11111111111 & 0001010110 \\

\bottomrule
\end{tabular}


==> tables/golomb_zeta.tex <==
\begin{tabular}{c llll}
\toprule

$x$ & $\enc{G}{x}{2}$ & $\enc{G}{x}{5}$ & $\enc{Z}{x}{2}$ & $\enc{Z}{x}{3}$ \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}

1 & \bit{0.0}    & \bit{0.00}  & \bit{0.00}    & \bit{0.00} \\
2 & \bit{0.1}    & \bit{0.01}  & \bit{0.10}    & \bit{0.010} \\
3 & \bit{10.0}   & \bit{0.10}  & \bit{0.11}    & \bit{0.011} \\
4 & \bit{10.1}   & \bit{0.110} & \bit{10.000}  & \bit{0.100} \\
5 & \bit{110.0}  & \bit{0.111} & \bit{10.001}  & \bit{0.101} \\
6 & \bit{110.1}  & \bit{10.00} & \bit{10.010}  & \bit{0.110} \\
7 & \bit{1110.0} & \bit{10.01} & \bit{10.011}  & \bit{0.111} \\
8 & \bit{1110.1} & \bit{10.10} & \bit{10.1000} & \bit{10.00000} \\

\bottomrule
\end{tabular}


==> tables/gov2.entropy.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $17.13$ & $23.72$\\

$512$ & $16.38$ & $22.67$\\

$1024$ & $16.27$ & $22.52$\\

$2048$ & $16.12$ & $22.32$\\

$4096$ & $15.89$ & $22.00$\\

$8192$ & $15.65$ & $21.66$\\

$16384$ & $15.35$ & $21.25$\\

$32768$ & $14.98$ & $20.74$\\
\bottomrule
\end{tabular}


==> tables/gov2.entropy.freqs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $1.80$ & $2.49$\\

$512$ & $1.76$ & $2.43$\\

$1024$ & $1.75$ & $2.42$\\

$2048$ & $1.74$ & $2.41$\\

$4096$ & $1.72$ & $2.39$\\

$8192$ & $1.71$ & $2.36$\\

$16384$ & $1.68$ & $2.33$\\

$32768$ & $1.65$ & $2.29$\\
\bottomrule
\end{tabular}


==> tables/gov2.gaps_entropy.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $2.75$ & $3.81$\\

$512$ & $2.22$ & $3.07$\\

$1024$ & $2.17$ & $3.00$\\

$2048$ & $2.11$ & $2.92$\\

$4096$ & $2.01$ & $2.78$\\

$8192$ & $1.92$ & $2.66$\\

$16384$ & $1.82$ & $2.52$\\

$32768$ & $1.71$ & $2.37$\\
\bottomrule
\end{tabular}


==> tables/gov2.gaps_logs.docs.tex <==
\begin{tabular}{rrr}
\toprule

min. len. 
& GB 
& bpi \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 


$0$ & $1.39$ & $1.92$\\

$512$ & $1.02$ & $1.41$\\

$1024$ & $0.99$ & $1.37$\\

$2048$ & $0.96$ & $1.32$\\

$4096$ & $0.90$ & $1.25$\\

$8192$ & $0.85$ & $1.18$\\

$16384$ & $0.80$ & $1.10$\\

$32768$ & $0.74$ & $1.02$\\
\bottomrule
\end{tabular}


==> tables/gov2.space.tex <==
\begin{tabular}{lrrrrrr}
\toprule

& \multicolumn{2}{@{}c@{}}{\textsf{space}} 
& \multicolumn{2}{@{}c@{}}{{\docs}} 
& \multicolumn{2}{@{}c@{}}{{\freqs}} \\

& \multicolumn{2}{@{}c@{}}{[{\total}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} \\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

{\bic}& $4.30$ & & $3.80$ & & $2.14$ & \\

\cmidrule(lr){2-7}

{\pef}
& $4.65$ & \color{DarkGray}{$(+8\%)$}
& $4.10$ & \color{DarkGray}{$(+8\%)$}
& $2.38$ & \color{DarkGray}{$(+11\%)$}\\

%{\CPEF}
%& $4.43$ & \color{DarkGray}{$(+3\%)$}
%& $3.81$ & \color{DarkGray}{$(+0\%)$}
%& $2.37$ & \color{DarkGray}{$(+10\%)$}\\
%
%{\ans}
%& $4.17$ & \color{DarkGray}{$(-3\%)$}
%& $3.96$ & \color{DarkGray}{$(+4\%)$}
%& $1.85$ & \color{DarkGray}{$(-13\%)$}\\

{\pfor}
& $4.96$ & \color{DarkGray}{$(+15\%)$}
& $4.48$ & \color{DarkGray}{$(+18\%)$}
& $2.38$ & \color{DarkGray}{$(+11\%)$}\\

{\cgamma}
& $5.58$ & \color{DarkGray}{$(+30\%)$}
& $5.08$ & \color{DarkGray}{$(+34\%)$}
& $2.63$ & \color{DarkGray}{$(+23\%)$}\\

{\cdelta}
& $5.56$ & \color{DarkGray}{$(+29\%)$}
& $4.79$ & \color{DarkGray}{$(+26\%)$}
& $2.90$ & \color{DarkGray}{$(+35\%)$}\\

{\simplee}
& $6.36$ & \color{DarkGray}{$(+48\%)$}
& $5.53$ & \color{DarkGray}{$(+46\%)$}
& $3.27$ & \color{DarkGray}{$(+53\%)$}\\

{\simplen}
& $6.23$ & \color{DarkGray}{$(+45\%)$}
& $5.55$ & \color{DarkGray}{$(+46\%)$}
& $3.07$ & \color{DarkGray}{$(+43\%)$}\\

{\simples}
& $5.96$ & \color{DarkGray}{$(+39\%)$}
& $5.34$ & \color{DarkGray}{$(+41\%)$}
& $2.91$ & \color{DarkGray}{$(+36\%)$}\\

{\qmx}
& $6.77$ & \color{DarkGray}{$(+57\%)$}
& $6.00$ & \color{DarkGray}{$(+58\%)$}
& $3.37$ & \color{DarkGray}{$(+57\%)$}\\

{\vb}
& $12.64$ & \color{DarkGray}{$(+194\%)$}
& $9.53$ & \color{DarkGray}{$(+151\%)$}
& $8.02$ & \color{DarkGray}{$(+274\%)$}\\

{\optvb}
& $5.68$ & \color{DarkGray}{$(+32\%)$}
& $4.87$ & \color{DarkGray}{$(+28\%)$}
& $3.04$ & \color{DarkGray}{$(+42\%)$}\\

{\varigb}
& $15.06$ & \color{DarkGray}{$(+250\%)$}
& $11.15$ & \color{DarkGray}{$(+194\%)$}
& $9.77$ & \color{DarkGray}{$(+356\%)$}\\

{\varigiu}
& $14.00$ & \color{DarkGray}{$(+225\%)$}
& $10.43$ & \color{DarkGray}{$(+175\%)$}
& $9.00$ & \color{DarkGray}{$(+320\%)$}\\

\bottomrule
\end{tabular}


==> tables/leftmost.tex <==
\begin{tabular}{ccccccccccccc}
\toprule

0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\

\cmidrule(lr){1-13}

-- & -- & -- & \textbf{\bit{0}} & \textbf{\bit{1}} & \textbf{\bit{0}} & \textbf{\bit{1}} & \textbf{\bit{0}} & \textbf{\bit{1}} & \textbf{\bit{0}} & \textbf{\bit{1}} & \textbf{\bit{0}} & \textbf{\bit{1}} \\
\bit{0} & \bit{0} & \bit{0} & \bit{0} & \bit{0} & \bit{1} & \bit{1} & \bit{1} & \bit{1} & \bit{1} & \bit{1} & \bit{1} & \bit{1} \\
\bit{0} & \bit{0} & \bit{1} & \bit{1} & \bit{1} & \bit{0} & \bit{0} & \bit{0} & \bit{0} & \bit{1} & \bit{1} & \bit{1} & \bit{1} \\
\bit{0} & \bit{1} & \bit{0} & \bit{1} & \bit{1} & \bit{0} & \bit{0} & \bit{1} & \bit{1} & \bit{0} & \bit{0} & \bit{1} & \bit{1} \\

\bottomrule
\end{tabular}


==> tables/next_geq_queries.tex <==
\begin{tabular}{c rrr l rrr l rrr}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 252 & 226 & 308
&
& 255 & 226 & 279
&
& 197 & 181 & 243
\\

{\uniform}
& 187 & 122 & 250
&
& 146 & 155 & 175
&
& 91 & 113 & 120
\\

{\interp}
& 955 & 897 & 1385
&
& 951 & 1012 & 1290
&
& 710 & 878 & 1100
\\

{\opt}
& 167 & 182 & 229
&
& 138 & 157 & 144
&
& 94 & 118 & 89
\\

{\roar}
& 115 & 137 & 185
&
& 90 & 119 & 133
&
& 55 & 80 & 82
\\

{\roaropt}
& 105 & 138 & 188
&
& 80 & 115 & 136
&
& 50 & 72 & 85
\\

{\slice}
& 145 & 174 & 225
&
& 90 & 110 & 134
&
& 48 & 57 & 69
\\

\bottomrule
\end{tabular}

==> tables/or_queries.tex <==
\begin{tabular}{c rrr l rrr l rrr}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 7754 & 12480 & 21000
&
& 2173 & 3924 & 6191
&
& 285 & 920 & 1407
\\

{\uniform}
& 9540 & 17952 & 29600
&
& 2704 & 5495 & 8589
&
& 366 & 1300 & 2000
\\

{\interp}
& 21115 & 39190 & 63972
&
& 6369 & 12898 & 20408
&
& 899 & 3185 & 5042
\\

{\opt}
& 8900 & 17000 & 28349
&
& 2560 & 5230 & 8300
&
& 350 & 1252 & 1887
\\

{\roar}
& 1737 & 3570 & 5001
&
& 562 & 1360 & 1762
&
& 80 & 356 & 543
\\

{\roaropt}
& 1950 & 4215 & 5180
&
& 638 & 1657 & 1812
&
& 86 & 408 & 551
\\

{\slice}
& 1955 & 4040 & 7440
&
& 590 & 1315 & 2265
&
& 73 & 276 & 476
\\

\bottomrule
\end{tabular}

==> tables/rice.gov2.space.tex <==
\begin{tabular}{lrrrrrr}
\toprule

& \multicolumn{2}{@{}c@{}}{\textsf{space}} 
& \multicolumn{2}{@{}c@{}}{{\docs}} 
& \multicolumn{2}{@{}c@{}}{{\freqs}} \\

& \multicolumn{2}{@{}c@{}}{[{\total}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} \\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

$\rice_4$& $8.76$ & & $6.99$ & & $5.16$ & \\

\cmidrule(lr){2-7}

$\rice_3$
& $7.67$ & \color{DarkGray}{$(-12\%)$}
& $6.31$ & \color{DarkGray}{$(-10\%)$}
& $4.32$ & \color{DarkGray}{$(-16\%)$}\\

$\rice_2$
& $6.75$ & \color{DarkGray}{$(-23\%)$}
& $5.71$ & \color{DarkGray}{$(-18\%)$}
& $3.64$ & \color{DarkGray}{$(-29\%)$}\\

$\rice_1$
& $6.02$ & \color{DarkGray}{$(-31\%)$}
& $5.20$ & \color{DarkGray}{$(-26\%)$}
& $3.12$ & \color{DarkGray}{$(-40\%)$}\\

\bottomrule
\end{tabular}


==> tables/space.tex <==
\begin{tabular}{c SSS l SSS l SSS}
\toprule

Method
& \multicolumn{3}{c}{$d = 10^{-2}$}
&
& \multicolumn{3}{c}{$d = 10^{-3}$}
&
& \multicolumn{3}{c}{$d = 10^{-4}$}
\\

\cmidrule(lr){1-1}
\cmidrule(lr){2-4}
\cmidrule(lr){6-8}
\cmidrule(lr){10-12}

& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
&
& {\gov} & {\clue} & {\cc}
\\

\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){10-10}
\cmidrule(lr){11-11}
\cmidrule(lr){12-12}

{\vb}
& 8.59874 & 8.72134 & 8.66218
&
& 8.71601 & 9.00413 & 9.07528
&
& 8.84851 & 9.18816 & 9.2832
\\

{\uniform}
& 2.72358 & 4.4415 & 4.71734
&
& 3.24897 & 5.14416 & 5.365
&
& 3.65433 & 5.56265 & 5.65584
\\

{\interp}
& 2.33174 & 3.58972 & 4.37232
&
& 2.72138 & 4.11178 & 4.96699
&
& 3.01666 & 4.40728 & 5.23847
\\

{\opt}
& 2.36912 & 4.00844 & 4.5165
&
& 2.84603 & 4.61834 & 5.15798
&
& 3.20086 & 4.96094 & 5.44576
\\

{\roar}
& 6.003608 & 8.881072 & 8.252430
&
& 7.02780 & 9.98834 & 9.21168
&
& 7.601203 & 10.474733 & 9.525385
\\

{\roaropt}
& 5.331765 & 8.494709 & 8.216347
&
& 6.245421 & 9.402477 & 9.169742
&
& 6.745314 & 9.751545 & 9.480298
\\

{\slice}
& 3.23281 & 5.4384 & 5.97909
&
& 3.91038 & 6.39024 & 7.1822
&
& 4.45539 & 7.00042 & 7.76609
\\

\bottomrule
\end{tabular}

==> tables/zeta.gov2.space.tex <==
\begin{tabular}{lrrrrrr}
\toprule

& \multicolumn{2}{@{}c@{}}{\textsf{space}} 
& \multicolumn{2}{@{}c@{}}{{\docs}} 
& \multicolumn{2}{@{}c@{}}{{\freqs}} \\

& \multicolumn{2}{@{}c@{}}{[{\total}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} 
& \multicolumn{2}{@{}c@{}}{[\textsf{bpi}]} \\

\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 

$\zeta_4$& $8.00$ & & $6.43$ & & $4.65$ & \\

\cmidrule(lr){2-7}

$\zeta_3$
& $6.88$ & \color{DarkGray}{$(-14\%)$}
& $5.71$ & \color{DarkGray}{$(-11\%)$}
& $3.81$ & \color{DarkGray}{$(-18\%)$}\\

$\zeta_2$
& $5.95$ & \color{DarkGray}{$(-26\%)$}
& $5.14$ & \color{DarkGray}{$(-20\%)$}
& $3.08$ & \color{DarkGray}{$(-34\%)$}\\

$\zeta_1$
& $5.58$ & \color{DarkGray}{$(-30\%)$}
& $5.08$ & \color{DarkGray}{$(-21\%)$}
& $2.63$ & \color{DarkGray}{$(-43\%)$}\\

\bottomrule
\end{tabular}

